Online Aggregation of Trajectory Predictors

Trajectory prediction, the task of forecasting future agent behavior from past data, is central to safe and efficient autonomous driving. A diverse set of methods (e.g., rule-based or learned with different architectures and datasets) have been proposed, yet it is often the case that the performance of these methods is sensitive to the deployment environment (e.g., how well the design rules model the environment, or how accurately the test data match the training data). Building upon the principled theory of online convex optimization but also going beyond convexity and stationarity, we present a lightweight and model-agnostic method to aggregate different trajectory predictors online. We propose treating each individual trajectory predictor as an "expert" and maintaining a probability vector to mix the outputs of different experts. Then, the key technical approach lies in leveraging online data -- the true agent behavior to be revealed at the next timestep -- to form a convex-or-nonconvex, stationary-or-dynamic loss function whose gradient steers the probability vector towards choosing the best mixture of experts. We instantiate this method to aggregate trajectory predictors trained on different cities in the NUSCENES dataset and show that it performs just as well, if not better than, any singular model, even when deployed on the out-of-distribution LYFT dataset.

==> sections/alg-discounted-squint.tex <==
%!TEX root = ../root.tex
\begin{algorithm}[hbt!]
\SetKwInput{KwInput}{Input}
\SetKwInput{KwInit}{Initialize}
\caption{Discounted \squint with Cutkosky Clipping}\label{alg:discounted-squint}
\KwInput{A prior distribution of the weights $\alpha_1$ for each expert, a discount factor $\lambda \leq 1$ }
\KwInit{Cumulative regret $R_1=0$, Cumulative regret squared $V_1=0$}
\For{$t=1,2,\dots, T$}{
    Obtain $\ell_t$ from the experts and define the gradient $\tilde{g}_t = \nabla_{\alpha_t}(\ell_t)$ 
    
    Set $G_t = \max (\max(|\tilde{g}_t|), G_{t-1})$, where ``$|\cdot|$'' and ``$\max$'' are applied element-wise \alex{How is max applied element wise? Shouldn't it be taking the max of the vector?}
    
    Define the clipped gradient $g_t = \frac{(\tilde{g}_t / G_t) + 1}{2}$ (element-wise division)
    
    Define the instantaneous regret $r_t = \alpha_t \cdot g_t - g_t$ (element-wise multiplication) \hy{@Alex, I am confused, is $r_t$ a scalar or a vector?} \alex{$r_t$ is a vector, basically each expert $i$ has their own $r^i_t, R^i_t$ and $V^i_t$}
    
    Update 
    \bea\label{eq:squint-update-alpha}
    \alpha_{t+1} = \frac{\alpha_1 \xi(R_t, V_t)}{\sum_i \alpha_1 \xi(R^i_t, V^i_t)}
    \eea
    where $\alpha_1 \xi(R_t, V_t)$ denotes the scalar multiplication of $\alpha_1$ and $\xi(R_t,V_t)$,
    \bea\label{eq:squint-error-function}
    \xi(R,V) = \sqrt{\pi} \exp{\left( \frac{R^2}{4V}\right)} \frac{\text{erfc}(\frac{-R}{2\sqrt{V}})-\text{erfc}(\frac{V-R}{2\sqrt{V}})}{2\sqrt{V}}
    \eea
    and erfc is the complementary error function $\text{erfc}(x) := 1 - \text{erf}(x) = 1 - \frac{2}{\sqrt{\pi}} \int_0^x e^{-t^2} dt$
    
    Update $R_{t+1} = \lambda R_{t} + r_t$ and $V_{t+1} = \lambda V_{t} + r_t^2$ \label{line:discounted-updateRV}
}
\end{algorithm}
